EvoJAX: Hardware-Accelerated Neuroevolution

Evolutionary computation has been shown to be a highly effective method for training neural networks, particularly when employed at scale on CPU clusters. Recent work have also showcased their effectiveness on hardware accelerators, such as GPUs, but so far such demonstrations are tailored for very specific tasks, limiting applicability to other domains. We present EvoJAX, a scalable, general purpose, hardware-accelerated neuroevolution toolkit. Building on top of the JAX library, our toolkit enables neuroevolution algorithms to work with neural networks running in parallel across multiple TPU/GPUs. EvoJAX achieves very high performance by implementing the evolution algorithm, neural network and task all in NumPy, which is compiled just-in-time to run on accelerators. We provide extensible examples of EvoJAX for a wide range of tasks, including supervised learning, reinforcement learning and generative art. Since EvoJAX can find solutions to most of these tasks within minutes on a single accelerator, compared to hours or days when using CPUs, our toolkit can significantly shorten the iteration cycle of evolutionary computation experiments. EvoJAX is available at https://github.com/google/evojax

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> figures/fig-examples-vertical01.tex <==
\begin{figure}[!ht]
\centering

\centering        
\includegraphics[width=0.4\textwidth]{figures/examples_vertical01.pdf}       
\caption{[Vertical layout test #1] EvoJAX examples. A) MNIST classification. B) Seq2Seq learning. C) Robotic control. D) Cart-pole swing up. E) Left: WaterWorld wherein the agent (yellow) tries to get food (green) while avoiding poison (red). Right: MultiAgentsWaterWorld with which we demonstrate multi-agent training. F) Abstract painting with only triangles. Left: Painting a concrete image. Right: Painting the concept ``Walt Disney World''.}
\label{fig:examples_vertical01} 
\vspace{-0.1in}

\end{figure}

==> figures/fig-examples.tex <==
\begin{figure*}[!ht]
\centering

\centering        
\includegraphics[width=1\textwidth]{figures/examples.pdf}       
\caption{EvoJAX examples. A) MNIST classification. B) Seq2Seq learning. C) Robotic control. D) Cart-pole swing up. E) Left: WaterWorld wherein the agent (yellow) tries to get food (green) while avoiding poison (red). Right: MultiAgentsWaterWorld with which we demonstrate multi-agent training. F) Abstract painting with only triangles. Left: Painting a concrete image. Right: Painting the concept ``Walt Disney World''.}
\label{fig:examples} 

\end{figure*}

==> submission_1-macro.tex <==
\AtBeginDocument{%
\providecommand\BibTeX{{%
\normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

\title{EvoJAX: Hardware-Accelerated Neuroevolution}

\author{Yujin Tang}
\email{yujintang@google.com}
\affiliation{%
  \institution{Google Brain}}

\author{Yingtao Tian}
\email{alantian@google.com}
\affiliation{%
  \institution{Google Brain}}

\author{David Ha}
\email{hadavid@google.com}
\affiliation{%
  \institution{Google Brain}}

\renewcommand{\shortauthors}{Yujin Tang, Yingtao Tian and David Ha}

\hypersetup{
colorlinks=true,linkcolor=blue
}

\definecolor{LightGray}{gray}{0.95}
\newenvironment{code}{\captionsetup{type=listing}}{}
